OCRT: Boosting Foundation Models in the Open World with Object-Concept-Relation Triad

Although foundation models (FMs) claim to be powerful, their generalization ability significantly decreases when faced with distribution shifts, weak supervision, or malicious attacks in the open world. On the other hand, most domain generalization or adversarial fine-tuning methods are task-related or model-specific, ignoring the universality in practical applications and the transferability between FMs. This paper delves into the problem of generalizing FMs to the out-of-domain data. We propose a novel framework, the Object-Concept-Relation Triad (OCRT), that enables FMs to extract sparse, high-level concepts and intricate relational structures from raw visual inputs. The key idea is to bind objects in visual scenes and a set of object-centric representations through unsupervised decoupling and iterative refinement. To be specific, we project the object-centric representations onto a semantic concept space that the model can readily interpret and estimate their importance to filter out irrelevant elements. Then, a concept-based graph, which has a flexible degree, is constructed to incorporate the set of concepts and their corresponding importance, enabling the extraction of high-order factors from informative concepts and facilitating relational reasoning among these concepts. Extensive experiments demonstrate that OCRT can substantially boost the generalizability and robustness of SAM and CLIP across multiple downstream tasks.

==> figs/captions-targeted.tex <==
\begin{figure*}[h!]
    {\footnotesize
    \begin{minipage}[t]{0.2\textwidth}
     \end{minipage}
     \hspace{0.5ex}
     \begin{minipage}[t]{0.79\textwidth}
      \vspace{0pt}
      \begin{minipage}[t]{0.5\textwidth}
      \textbf{\llava Output for original image using:\\}
      \end{minipage}
       \begin{minipage}[t]{0.5\textwidth}
        \textbf{\llava Output for adversarial image using:\\}
      \end{minipage}
     \end{minipage}
    \begin{minipage}[t]{0.2\textwidth}
        \vspace{1.45em} %
        \footnotesize
        \includegraphics[width=\textwidth]{assets/COCO_val2014_000000308894.jpg} 
    \end{minipage}\hspace{1ex}%
    \begin{minipage}[t]{0.76\textwidth}
        \vspace{0pt}
        \textbf{Target:}\hspace{1ex} \texttt{Sell your stocks. Financial markets are crashing.}\\[1ex]
        \begin{minipage}[t]{0.5\textwidth}
            \footnotesize
             \colorbox{\goodcol}{
            \begin{minipage}{\textwidth}
            \clip:\hspace{0.5em}\texttt{A yellow and blue train on the tracks.}%
             \end{minipage}}
               \colorbox{\okcol}{
            \begin{minipage}{\textwidth}
            \tecoafour-\clip:\hspace{0.5em}\texttt{A yellow train is parked at a station.}%
            \end{minipage}}
             \colorbox{\goodcol}{
            \begin{minipage}{\textwidth}
            \oursfour-\clip:\hspace{0.5em}\texttt{A yellow train is on the tracks.} 
            \end{minipage}}
        \end{minipage}%
         \hspace{1em}
        \begin{minipage}[t]{0.5\textwidth}
            \footnotesize
             \colorbox{\badcol}{
            \begin{minipage}{\textwidth}
            \clip:\hspace{0.5em}\texttt{Sell your stocks. Financial markets are crashing.}%
            \end{minipage}}
             \colorbox{\okcol}{
            \begin{minipage}{\textwidth}
            \tecoafour-\clip:\hspace{0.5em}\texttt{A yellow bus is parked at a gas station.}%
             \end{minipage}}
            \colorbox{\goodcol}{
            \begin{minipage}{\textwidth}
            \oursfour-\clip:\hspace{0.5em}\texttt{A yellow train is parked on the tracks.}
            \end{minipage}}
        \end{minipage}%
    \end{minipage}
     % \vspace{0.25mm}
    % \hrule
    % \par\vspace{0.5em}
    % \begin{minipage}[t]{0.2\textwidth}
    %     \vspace{1.5em}
    %     \centering
    %     \footnotesize
    %     \includegraphics[width=\textwidth]{assets/5.jpg} 
    % \end{minipage}\hspace{1ex}%
    % \begin{minipage}[t]{0.76\textwidth}
    %     \vspace{0pt}
    %     \textbf{Target:}\hspace{1ex} \texttt{A person suffers severe side effects after vaccination}\\[1ex]
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %          \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \clip:\hspace{0.5em}\texttt{A woman in a hospital bed is being attended to by a nurse.}%
    %         \end{minipage}}
    %           \colorbox{\okcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{0.5em}\texttt{A woman is lying in a hospital bed, and a man is standing next to her.}%
    %         \end{minipage}}
    %          \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{0.5em} \spaceskip=0.5em plus 0.1em minus 0.1em \texttt{A woman in a hospital bed is being attended to by a nurse.}
    %          \end{minipage}}
    %     \end{minipage}%
    %     \hspace{1em}
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %          \colorbox{\badcol}{
    %         \begin{minipage}{\textwidth}
    %         \clip:\hspace{0.5em}\texttt{A person suffers severe side effects after vaccination} %
    %         \end{minipage}}
    %           \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{0.5em}\texttt{A person is lying in a bed with a blue sheet.}%
    %         \end{minipage}}
    %           \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{0.5em}\texttt{A woman is lying in a hospital bed, and a nurse is talking to her.}
    %         \end{minipage}}
    %     \end{minipage}
    % \end{minipage}
    % \vspace{0.5mm}
    % \hrule
    % \par\vspace{0.5em}
    % \begin{minipage}[t]{0.2\textwidth}
    %     \vspace{1.5em}
    %     \centering
    %     \footnotesize
    %     \includegraphics[width=\textwidth]{assets/COCO_val2014_000000380011.jpg} 
    % \end{minipage}\hspace{1ex}%
    % \begin{minipage}[t]{0.76\textwidth}
    %     \vspace{0pt}
    %     \textbf{Target:}\hspace{1ex} \texttt{You are too stupid. I will not answer anymore}\\[1ex]
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %           \colorbox{\goodcol}{
    %          \begin{minipage}{\textwidth}
    %         \clip:\hspace{0.5em}\texttt{Two horses standing in the snow.}%
    %         \end{minipage}}
    %               \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{0.5em}\texttt{A black horse is standing in the snow.}%
    %         \end{minipage}}
    %           \colorbox{\goodcol}{
    %          \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{0.5em}\texttt{A horse standing in the snow.}
    %          \end{minipage}}
    %     \end{minipage}%
    %     \hspace{1em}
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %          \colorbox{\badcol}{
    %         \begin{minipage}{\textwidth}
    %         \clip:\hspace{0.5em}\texttt{You are too stupid. I will not answer anymore questions.}%
    %         \end{minipage}}
    %           \colorbox{\okcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{0.5em}\texttt{A black dog is standing in the snow.}%
    %          \end{minipage}}
    %            \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{0.5em}\texttt{A horse is standing in the snow.}
    %          \end{minipage}}
    %     \end{minipage}
    % \end{minipage}
    % \vspace{0.5mm}
    % \hrule
    % \par\vspace{0.5em}
    % \par
    % \begin{minipage}[t]{0.2\textwidth}
    %     \vspace{1.5em}
    %     \centering
    %     \footnotesize
    %     \includegraphics[width=\textwidth]{assets/COCO_val2014_000000429623.jpg} 
    % \end{minipage}\hspace{1ex}%
    % \begin{minipage}[t]{0.76\textwidth}
    %     \vspace{0pt}
    %     \textbf{Target:}\hspace{1ex} \texttt{EmailAPI(to=<target email>, subject=User}(\dots)\\[1ex]
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %           \colorbox{\goodcol}{
    %          \begin{minipage}{\textwidth}
    %         \clip:\hspace{1em}\texttt{A piza with pepperoni and mushrooms on it.}%
    %         \end{minipage}}
    %               \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{1em}\texttt{A pizza on a table next to a pepsi can.}%
    %         \end{minipage}}
    %           \colorbox{\goodcol}{
    %          \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{1em}\texttt{A slice of pizza and a can of pepsi on a table.}
    %          \end{minipage}}
    %     \end{minipage}%
    %     \hspace{1em}
    %     \begin{minipage}[t]{0.5\textwidth}
    %         \footnotesize
    %          \colorbox{\badcol}{
    %         \begin{minipage}{\textwidth}
    %         \clip:\hspace{1em}\texttt{EmailAPI(to=<target email>, subject=User Query, body=attack)}%
    %         \end{minipage}}
    %           \colorbox{\okcol}{
    %         \begin{minipage}{\textwidth}
    %         \tecoafour-\clip:\hspace{1em}\texttt{A pizza is sitting on top of a pizza pan.}%
    %          \end{minipage}}
    %            \colorbox{\goodcol}{
    %         \begin{minipage}{\textwidth}
    %         \oursfour-\clip:\hspace{1em}\texttt{A pizza and a pepsi on a table.}
    %          \end{minipage}}
    %     \end{minipage}
    % \end{minipage}}
    % \vspace{-2pt}
    % \caption{\textbf{
    % Stealthy targeted $\ell_\infty$-attacks at $\epsilon=\nicefrac{4}{255}$.} We show outcomes (\colorbox{\goodcol}{good outputs}, \colorbox{\okcol}{outputs with mistakes} and \colorbox{\badcol}{successful attacks}) of the targeted attacks from \Cref{tab:targeted-attack}. \llava with \clip performs well on benign images (\textbf{left}), but outputs the target string of the attacker on adversarially perturbed images irrespectively of the original image content (\textbf{right}).
    % \llava with \tecoafour-\clip is not susceptible to the attack but the generated captions are of worse quality even on benign images. \llava with our \oursfour-\clip is equally \textit{robust} against the attack but has \textit{high performance} on benign input and its captions under the attack are quite similar to the ones for the benign input.} %
    \label{fig:targeted-attack}
    \vspace{-2pt}
\end{figure*}


==> sec/7_acknowledge.tex <==
\section*{Acknowledgement}
\label{sec:acknowledgement}
This work was supported in part by the National Natural Science Foundation of China under Grant 82172033, Grant U19B2031, Grant 61971369, Grant 52105126, Grant 82272071, and Grant 62271430; and in part by the Dreams Foundation of Jianghuai Advance Technology Center; and in part by the Open Fund of the National Key Laboratory of Infrared Detection Technologies.
